UniMoCo: Unified Modality Completion for Robust Multi-Modal Embeddings

Current vision-language models have been explored for multi-modal embedding tasks like information retrieval. However, they face significant challenges in real-world queries and targets involving diverse modality combinations, as existing approaches often fail to align all modality combinations within a unified embedding space during training, leading to degraded performance on rare modality patterns during inference. To address this fundamental limitation, we propose UniMoCo, a novel architecture featuring a modality-completion module that generates visual features from text, thereby ensuring modality completeness for both queries and targets. Additionally, UniMoCo incorporates a specialized training strategy that aligns embeddings from both original and modality-completed inputs, thus ensuring consistent and robust embeddings for diverse modality combinations. Comprehensive experiments demonstrate that UniMoCo outperforms previous methods while exhibiting consistent robustness across diverse settings. Furthermore, we identify and quantify the inherent bias in conventional approaches caused by imbalanced modality combinations in training data, showing that our modality-completion paradigm effectively mitigates this limitation. The code is available at https://github.com/HobbitQia/UniMoCo.

==> setting-ai.tex <==
% =============================================================
%         setting for AI paper
%
%   Author      : Bei Yu
%   Last Update : 04/2025
% =============================================================

\usepackage[utf8]{inputenc}                         % allow utf-8 input
\usepackage[T1]{fontenc}                            % use 8-bit T1 fonts
\usepackage{microtype}                              % microtypography
\usepackage{natbib}
\usepackage{color}
\usepackage{xcolor,colortbl}                        % textcolor
\usepackage{longtable}
\usepackage{booktabs}                               % professional-quality tables
\usepackage{makecell}
\usepackage[export]{adjustbox}
\usepackage{multirow}
\usepackage{paralist}                               % compactitem
% \usepackage{cite}                                 % more citations in one bracket
\usepackage{comment}                                % use comment
\usepackage{soul}                                   % use highlight command \hl{}
\soulregister\cite7
\soulregister\ref7
\soulregister\pageref7
\usepackage{enumerate}
\usepackage{url}
\usepackage{nth}                                    % nth command
\usepackage{courier}
\usepackage{balance}
\usepackage{threeparttable}
\usepackage{footnote}
\usepackage{listings}
\usepackage{setspace}                               % setstretch{}
\usepackage[inline]{enumitem}
\usepackage{verbatim}
\usepackage{etoolbox}                               % commands \newtoggle, \toggletrue, \iftoggle
\usepackage[bookmarks=false]{hyperref}
\hypersetup{
    colorlinks = true,
    citecolor  = blue,
    linkcolor  = blue,
    urlcolor   = blue,
}
\usepackage{pifont}                                 % ding commend
\usepackage[figuresright]{rotating}
\usepackage{moresize}
\usepackage{fontawesome}

% ==================================================================
%                       math Packages
% ==================================================================
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{amsfonts}                               % blackboard math symbols
\usepackage{amsthm}
\usepackage[mathcal]{eucal}
\usepackage{mathrsfs}
\usepackage{bm}                                     % bm command
\usepackage{blkarray}                               % to support matrix
\usepackage{nicefrac}                               % compact symbols for 1/2, etc.

% ==================================================================
%                       subfigure Packages
% ==================================================================
\usepackage{wrapfig}
\usepackage{graphicx}                               % include pdf figures
\iffalse
\usepackage[subrefformat=parens,farskip=0pt,justification=centering]{subfig}
\else
\usepackage{subfigure}
\fi
\renewcommand\thesubfigure{(\alph{subfigure})}      % "Fig.~1b"-->"Fig.1(b)"
\usepackage{caption}
\captionsetup[table]{skip=2pt}
\captionsetup{labelsep=space}
\captionsetup[subfigure]{labelformat=simple}        % avoid "double brackets" in sub-figure caption
\usepackage{cleveref}
% \Crefformat{figure}{Fig.~#2#1#3}                    % "Fig.", instead of "Figure"
% \Crefname{subfigure}{Fig.}{Figs.}
% \Crefname{figure}{Fig.}{Figs.}
% \Crefformat{table}{TABLE~#2#1#3}                    % "TABLE", instead of "Table"

% ==================================================================
%                         tikz Packages
% ==================================================================
\usepackage{tikz}                                          
\usepackage{circuitikz}
\usetikzlibrary{patterns,snakes}
\usetikzlibrary{positioning,calc,fit,decorations.pathmorphing,shapes.geometric, shapes.gates.logic.US, calc}
\usetikzlibrary{arrows,arrows.meta,decorations.markings,shapes,shapes.arrows}
\usetikzlibrary{decorations,decorations.pathreplacing}
\usetikzlibrary{backgrounds}
\usepackage{filecontents}                           % support to pgfplots
\usepackage{pgfplots}
\usepackage{pgfplotstable}
\usepgfplotslibrary{groupplots}
\usepackage{scalefnt}
\pgfplotsset{compat=newest}

% ==================================================================
%                         Algorithm Packages
% ==================================================================
\usepackage{algorithm}
% ====== option 1: algpseudocode package
\iffalse
%\usepackage[noend]{algpseudocode}
\usepackage{algpseudocode}                          % new algorithm package
\algrenewcommand\textproc{\texttt}
\renewcommand{\algorithmicrequire}{\textbf{Input:}} % Use Input in the format of Algorithm
\renewcommand{\algorithmicensure}{\textbf{Output:}} % Use Output in the format of Algorithm
% long line in algorithm
% e.g.: \Statex[4] ...;
\makeatletter
\let\OldStatex\Statex
\renewcommand{\Statex}[1][3]{%
  \setlength\@tempdima{\algorithmicindent}%
  \OldStatex\hskip\dimexpr#1\@tempdima\relax
}
\makeatother
\else
% ====== option 2: algorithmic package
\usepackage{algorithmic}
\fi
\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator*{\argmax}{argmax}


% =============================================================
%                   Theorem Definitions
% =============================================================
\newtheorem{myproblem}{\textbf{Problem}}
\newtheorem{mydefinition}{\textbf{Definition}}
\newtheorem{mytheorem}{\textbf{Theorem}}
\newtheorem{mycorollary}{\textbf{Corollary}}
\newtheorem{mylemma}{\textbf{Lemma}}
\newtheorem{myclaim}{\textbf{Claim}}
\newtheorem{myapplication}{\textbf{Application}}
\newtheorem{myexample}{\textbf{Example}}
\newtheorem{myconjecture}{\textbf{Conjecture}}
\newtheorem{myassumption}{Assumption}
\newtheorem{myprop}{Property}

\crefname{mytheorem}{Theorem}{Theorems}
\crefname{mylemma}{Lemma}{Lemmas}
\crefname{myclaim}{Claim}{Claims}
\crefname{myproperty}{Property}{Properties}
\crefname{mycorollary}{Corollary}{Corollaries}


% ==================================================================
%                    Local news commands 
% ==================================================================
\newcommand{\etal}{\textit{et al.}}
\newcommand{\cbit}{\begin{compactitem}}
	\newcommand{\ceit}{\end{compactitem}}
\newcommand{\cben}{\begin{compactenum}}
	\newcommand{\ceen}{\end{compactenum}}
\newcommand{\calH}{\mathcal{H}}
\newcommand{\calL}{\mathcal{L}}
\newcommand{\calN}{\mathcal{N}}
\newcommand{\calO}{\mathcal{O}}
\newcommand{\calP}{\mathcal{P}}
\newcommand{\calQ}{\mathcal{Q}}
\newcommand{\calV}{\mathcal{V}}
\newcommand{\calKL}{\mathcal{KL}}
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\newcommand{\tool}[1]{$\mathsf{#1}$}
\newcommand{\tensor}[1]{\mathcal{#1}}      % define tensor command
\renewcommand{\vec}[1]{\boldsymbol{#1}}    % re-define vec command
\newcommand{\abs}[1]{\ensuremath{\left\lvert #1\right\rvert}}
\newcommand{\mathbbm}[1]{\text{\usefont{U}{bbm}{m}{n}#1}}
\newcommand{\minisection}[1]{\vspace{.1in}\noindent{\textbf{#1}}.}
\newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}}
\newcommand{\todo}[1]{\textcolor{red}{[TODO: #1]}}
\newcommand{\revise}[1]{\DIFadd{#1}}
\newcommand\blfootnote[1]{                 % footnote w/o. label
  \begingroup
  \renewcommand\thefootnote{}\footnote{#1}%
  \addtocounter{footnote}{-1}%
  \endgroup
}
\newcommand*\bcircled[1]{                  % black circled
    \tikz[baseline=(char.base)]{
        \node[shape=circle,fill,inner sep=1pt] (char) {\textcolor{white}{#1}};
    }
}
\newcommand*\wcircled[1]{                  % white circled
    {\textcircled{\scriptsize{\textbf{#1}}}}
}
% === beamer style block
\usepackage{tcolorbox}
\tcbuselibrary{skins,breakable}
\newenvironment{myblock}[1]{%
    \tcolorbox[beamer,%
    noparskip,breakable,
    colback=white,colframe=CUHKmiddle,%
    colbacklower=white,%
    title=#1]}%
    {\endtcolorbox}
%learn from ChatGPT, automatic add Comment.
\newenvironment{commentblock}[1]{%
    \tcolorbox[beamer,%
    noparskip,breakable,
    colback=white,colframe=CUHKmiddle,%
    colbacklower=white,%
    title=Comment #1]}%
    {\endtcolorbox}


% ==================================================================
%                    Local color definitions 
% ==================================================================
\definecolor{CUHKorange}{RGB}{244,106,18} %F47012
\definecolor{CUHKblue}{RGB}{0,111,190}    %006FBE
\definecolor{CUHKgreen}{RGB}{0,127,128}   %007F80
\definecolor{CUHKred}{RGB}{228,46,36}     %E42E24
\definecolor{CUHKyellow}{RGB}{198,148,34} %C69422
\definecolor{CUHKdark}{RGB}{114,44,114}   %722C72
\definecolor{CUHKmiddle}{RGB}{144,44,144} %902C90
\definecolor{CUHKlight}{RGB}{167,44,167} 
\definecolor{CUHKpurple}{RGB}{117,15,109}
\definecolor{CUHKgold}{RGB}{221,163,0}
\definecolor{CUHKribbon}{RGB}{244,223,176}
\definecolor{CUHKblack}{RGB}{34,24,21}




% =============================================================
%              page size setting 
% =============================================================
\iffalse
\paperwidth   = 8.5in                                      % US Letter
\paperheight  = 11.0in
%\paperwidth  = 8.26in                                     % A4
%\paperheight = 11.69in
\usepackage[top=0.80in,bottom=0.88in,left=0.63in,right=0.63in]{geometry}
\linespread{1.00}
\setlength{\columnsep}{20pt}                               % set space between columns
\setlength{\textfloatsep}{10pt plus 1pt minus 1pt}         % set space between float and text
\setlength{\floatsep}{10pt plus 1pt minus 1pt}             % set space between two floats
\setlength{\intextsep}{4pt plus 1pt minus 1pt}             % set space between text and float
\setlength{\abovecaptionskip}{2pt}                         % set space between figure and caption
\setlength{\belowcaptionskip}{2pt}                         % set space between figure and caption
% ==== reduce space around equations
\setlength{\belowdisplayskip}{4pt} \setlength{\belowdisplayshortskip}{4pt}
\setlength{\abovedisplayskip}{4pt} \setlength{\abovedisplayshortskip}{4pt}
% ==== reduce section and subsection title spacing
\newcommand{\subparagraph}{}
\usepackage{titlesec}
\titlespacing*{\section}{0pt}{1.8ex plus .2ex minus .2ex}{0.4ex plus .2ex}
\titlespacing*{\subsection}{0pt}{1.0ex plus .2ex minus .2ex}{0.2ex plus .2ex}
\fi


% ==== Logs:
%
%  04/2025: initilization, migrated from ieee template
%


